Reciprocal Learning

We demonstrate that a wide array of machine learning algorithms are specific instances of one single paradigm: reciprocal learning. These instances range from active learning over multi-armed bandits to self-training. We show that all these algorithms do not only learn parameters from data but also vice versa: They iteratively alter training data in a way that depends on the current model fit. We introduce reciprocal learning as a generalization of these algorithms using the language of decision theory. This allows us to study under what conditions they converge. The key is to guarantee that reciprocal learning contracts such that the Banach fixed-point theorem applies. In this way, we find that reciprocal learning algorithms converge at linear rates to an approximately optimal model under relatively mild assumptions on the loss function, if their predictions are probabilistic and the sample adaption is both non-greedy and either randomized or regularized. We interpret these findings and provide corollaries that relate them to specific active learning, self-training, and bandit algorithms.

==> old.tex <==


\section{Adaptive/Reciprocal Learning}




 \[
     f :
    \begin{cases}
      \Theta \times \mathcal{P} \times \mathbb N &\rightarrow \mathcal{P} \\
      (\theta_{t-1}, \mathbb P_{t-1}(Y , X), n_{t-1})  &\mapsto \mathbb P_t(Y , X),
    \end{cases}
    \]

    % \[\mathbb P(X = x) = \frac{\sum_{i=1}^n \mathbbm 1(x_i = x) + \sum_{i=n+1}^m \mathbbm 1(i \in S_{1:t}, x_i = x)}{n + |S_{1:t}|}\]
    where $\mathbb P_t(Y , X)$ is given by 
    \[\mathbb P_t(Y = 1 , X = x) = \frac{ 1(x = x(\theta_{t-1})) \cdot \hat y(x(\theta_{t-1}), \theta_{t-1})  + n_{t-1} \, \mathbb P_{t-1}(Y , X = x)) }{n_{t-1}+1} \]

    with one data point being added at a time.

    BZW mit gewichten: 
    \[\mathbb P_t(Y = 1 , X = x) = \frac{ 1(x = x(\theta_{t-1})) \cdot  y(x(\theta_{t-1}), \theta_{t-1}) \cdot w(\theta_{t-1}, x(\theta_{t-1})) + n_{t-1} \, \mathbb P_{t-1}(Y , X = x)) }{n_{t-1}+1} \]
    

\section{Active Learning}


 \[
     f :
    \begin{cases}
      \Theta \times \mathcal{P} \times \mathbb N &\rightarrow \mathcal{P} \\
      (\theta_{t-1}, \mathbb P_{t-1}(Y , X), n_{t-1})  &\mapsto \mathbb P_t(Y , X),
    \end{cases}
    \]

    % \[\mathbb P(X = x) = \frac{\sum_{i=1}^n \mathbbm 1(x_i = x) + \sum_{i=n+1}^m \mathbbm 1(i \in S_{1:t}, x_i = x)}{n + |S_{1:t}|}\]
    where $\mathbb P_t(Y , X)$ is given by 
    \[\mathbb P_t(Y = 1 , X = x) = \frac{ 1(x = x(\theta_{t-1})) \cdot  y(x(\theta_{t-1}), \theta_{t-1}) \cdot w(\theta_{t-1}, x(\theta_{t-1})) + n_{t-1} \, \mathbb P_{t-1}(Y , X = x)) }{n_{t-1}+1} \]

with continuous $x(\theta_{t-1})$ defined as follows and $ y(x(\theta_{t-1}), \theta_{t-1})$ is obtained by queries from an oracle. For self-training, replace  $ y(x(\theta_{t-1}), \theta_{t-1})$ by  $ \hat y(x(\theta_{t-1}), \theta_{t-1})$

\begin{definition}
    Define the following data selection function:
$$
x: 
    \begin{cases}
      \Theta &\rightarrow \mathcal{X} \\
      \theta &\mapsto \underset{\boldsymbol{x} \in \mathcal{X}}{\operatorname{argmax}}\left\{c(\boldsymbol{x}, \theta) + \frac{1}{L_s} R(\boldsymbol{x})\right\},
      \end{cases}
$$
where $c$ is some (linear?) criterion from the decision problem $(\Theta, \mathbb A, u_{\hat \theta_t})$, see TO DO, and $R(\cdot)$ is a $\kappa$-strongly convex regularizer.    \\

\end{definition}


==> possible-future-work.tex <==


\begin{theorem}[Strong Model Convergence Implies Weak Data Convergence]
    
\end{theorem}

\begin{proof}
    Assume reciprocal learning $R$ strongly converges to a model $\theta_c$ in the sense of definition~\ref{def-convergence}. That is, $\lim_{t \rightarrow \infty} \theta_t = \theta_{c}$. This implies a stationary data selection criterion $\tilde c$ (definition~\ref{def:data-select}) in the sense of $ \lim_{k,m \rightarrow \infty} \tilde c(x,\theta_k) = \tilde c(x,\theta_m)$. This in turn implies the stationarity of the maximizer of $\tilde c$. In case of deterministic data selection, we thus have $\lim_{k,m \rightarrow \infty}  x_d(\theta_{m}) = $  $x_d(\theta_{k})$. The Wasserstein-1-distance between two empirical distributions that share all $n$ instances except one is trivially upper bounded by any transport plan that moves probability mass $\frac{1}{n+1}$ from all $n$ instances to the one instance not being shared. (In our case of deterministic data selection, this instance is $x_d(\theta_{m}) = $  $x_d(\theta_{k})$, i.e., the same for both samples.) For this upper bound of the Wasserstein-1-distance it holds $\lim_{t \rightarrow \infty} \frac{1}{n(t)+1} = 0$, as $R$ adds one instance per iteratotion to the sample. The latter, however, holds anyway if $t$ and thus $n$ go to infinity.    
    
    In case of deterministic data selection, we also have $x_d(\theta_{m}) = $  $x_d(\theta_{k})$ and thus $\forall t: W_1(\mathbb P_t, \mathbb P_{t-1}) \leq W_1(\mathbb P_{t-1}, \mathbb P_{t-2})$, because the distance (on the support of $X,Y$; note that the potentially soft label for selected $x$ does not change, since our model does not change) of the newly added data point to all other existing data points does not change. We conclude that condition ii) in definition~\ref{def-convergence} is fulfilled.   
    
\end{proof}

The interpretation of this theorem is as follows. If reciprocal learning converges to a stable model $\theta_c$, the change in the sample oscillates within a given neighborhood. 

Frage: Ist die Umgebung von P ein credal set??




\textbf{Cybernetics:}Cybernetic? Lies Wiener!
https://www.nature.com/articles/s42256-019-0100-x
https://asc-cybernetics.org/definitions/
%




\textbf{Performative Reinforcement Learning:}
    TO DO \cite{mandal2023performative} introduce ....
Contrary to \cite{mandal2023performative}, we do not extend established methods to account for performativity. We rather show that \textit{existing} and well-established algorithms are instances of can be summarized as reciprocal learning of both data and parameters under the lense of performativity. Furthermore, \cite{mandal2023performative} address changing population quantities... TO DO

\textbf{Bayes Duality:} \cite{JMLR:v24:22-0291} Duality between $\mu$ and $\lambda$ (data and parameters? noch nicht verstanden)

Inference on Adaptively Collected Data \cite{zhang2023statistical}


related work: 

While we rely on similar techniques as in \cite{perdomo2020performative, miller2021outside}, namely Lipschitz-continuity and Wasserstein-distance, our work is conceptually different. Reciprocal learning deals with parameters altering the \textit{sample} (training data) at hand, while the population is fixed and, thus, the inference goal static. 

The technical part of this paper is inspired by TO DO charaterizations of convergence through contraction mappings .... TO DOperformatively stable repeated risk minimization in the context of performative prediction \cite{perdomo2020performative,mendler2020stochastic, miller2021outside, perf-power, hardt2023performative}. The concept refers to predictions that inform decision-makers triggering actions that influence the outcome that was aimed to be predicted in the first place. 


Repeated risk minimization is generally umimplementable in \cite{perdomo2020performative, mendler2020stochastic, miller2021outside, perf-power, hardt2023performative}, because the \textit{population} risk is being minimized. In this work, however, we are concerned with concrete, existing algorithms with an explicit mechanism of how the model (and its predictions) in $t$ affect the sample in $t+1$.    


In other words, reciprocal learning is an \textit{in sample} procedure, while continual learning describes reciprocal interactions  
However, unlike in reciprocal learning,  



OPTIONAL: (move to related work?) We might as well simply assume its Lipschitz-continuity, similar to performative prediction \cite{perdomo2020performative}, where a function $\mathcal{D}: \Theta \rightarrow \mathcal{P}$ describes the change of the population and is assumed to be (sufficiently) Lipschitz-continuous. Contrary to the population level, where such an assumptions is both inevitable and reasonable, however, we want to study changes in the sample induced by the algorithm \textit{directly}. In order to check concrete reciprocal learning algorithms such as active learning and the like for convergence, we need to define $f$ explicitly.          

